Kernel Angle Dependence Measures for Complex Objects

Measuring and testing dependence between complex objects is of great importance in modern statistics. Most existing work relied on the distance between random variables, which inevitably required the moment conditions to guarantee the distance is well-defined. Based on the geometry element ``angle", we develop a novel class of nonlinear dependence measures for data in metric space that can avoid such conditions. Specifically, by making use of the reproducing kernel Hilbert space equipped with Gaussian measure, we introduce kernel angle covariances that can be applied to complex objects such as random vectors or matrices. We estimate kernel angle covariances based on $U$-statistic and establish the corresponding independence tests via gamma approximation. Our kernel angle independence tests, imposing no-moment conditions on kernels, are robust with heavy-tailed random variables. We conduct comprehensive simulation studies and apply our proposed methods to a facial recognition task. Our kernel angle covariances-based tests show remarkable performances in dealing with image data.

==> definition.tex <==
\usepackage{latexsym, amsbsy, amssymb,multirow, epsfig, amsmath}
\usepackage{hyperref}

%--------------------Initialize---------------------%
%\textheight= 9in  \textwidth = 6.5in \topmargin = -1.4cm
%\oddsidemargin = -0.15in \evensidemargin = 0in
\usepackage{natbib,graphicx,setspace,lscape,longtable}
\usepackage{natbib,epsfig,graphicx}
\usepackage{subfigure}
%\usepackage{floatrow}   
\usepackage{tikz}
%\usepackage{subcaption}
\usepackage{xcolor} 
\usepackage[framemethod=tikz]{mdframed}
\usepackage{amsmath,amsthm,amssymb,color}
\RequirePackage[mathlines, displaymath]{lineno}
\bibpunct{(}{)}{;}{a}{,}{,}

\setlength{\textwidth}{6.2in} \setlength{\textheight}{8.75in}
\setlength{\topmargin}{-0.25in} \setlength{\oddsidemargin}{0.25in}
\setlength{\evensidemargin}{0.25in}
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
%\newtheorem{theorem}{Theorem}
%\newtheorem{lemma}{Lemma}
%\newtheorem{prop}{Proposition}
\baselineskip = 7mm
\parskip = 2.5mm

%\usepackage{titlesec} % for redefine section
%\titleformat{\section} % command
%{\centering\large\bfseries} % shape
%{\thesection.} % sep
%{0.5em} % before
%{} % after
%
%
%\titleformat{\subsection}
%{\centering\it%
%}
%{\thesubsection.} %sep
%{0.5em}{}


\newcommand{\csection}[1]
    {\begin{center}
        \stepcounter{section}
        {\bf\large\arabic{section}. #1}
    \end{center}
    \vspace{-0.15 cm}
}

\newcommand{\scsection}[1]
    {\begin{center}
        {\bf\large #1}
    \end{center}
    \vspace{-0.15 cm}
}

\newcommand{\csubsection}[1]{
\vspace{-0.25 cm}
\begin{center}
\stepcounter{subsection}
{\it\arabic{section}.\arabic{subsection}. #1}
\end{center}
\vspace{-0.25 cm}
}

\newcommand{\scsubsection}[1]{
\vspace{-0.25 cm}
\begin{center}
\stepcounter{subsection}
{\it #1}
\end{center}
\vspace{-0.25 cm}
}

\def\beqr{\begin{eqnarray}}
\def\eeqr{\end{eqnarray}}
\def\beqrs{\begin{eqnarray*}}
\def\eeqrs{\end{eqnarray*}}
\def\bep{\begin{prop}}
\def\eep{\end{prop}}

\def\mR{\mathbb{R}}
\def\calA{\mathcal{A}}
\def\calB{\mathcal{B}}
\def\calC{\mathcal{C}}
\def\calD{\mathcal{D}}
\def\calF{\mathcal{F}}
\def\calI{\mathcal{I}}
\def\calS{\mathcal{S}}
\def\calP{\mathcal{P}}
\def\calM{\mathcal{M}}
\def\calN{\mathcal{N}}
\def\calU{\mathcal{U}}
\def\calT{\mathcal{T}}
\def\calH{\mathcal{H}}
\def\calR{\mathcal{R}}
\def\calX{\mathcal{X}}
\def\calY{\mathcal{Y}}
\def\calZ{\mathcal{Z}}

%\newtheorem{Theorem}{Theorem}[section]
%\newtheorem{Corollary}{Theorem}[section]
%\newtheorem{Lemma}[Theorem]{Lemma}




\def\bias{\mbox{bias}}
\def\pr{\mbox{pr}}
\def\var{\mbox{var}}
\def\cov{\mbox{cov}}
\def\cor{\mbox{cor}}
\def\MSE{\mbox{MSE}}
\def\arcos{\mbox{arcos}}

\textheight= 9in
\textwidth = 6.1in
\evensidemargin = 0in
\renewcommand{\thefootnote}{\fnsymbol{footnote}}


\numberwithin{equation}{section}
\renewcommand{\baselinestretch}{1.75}


%\bibliographystyle{cheng}
%\renewcommand\refname{REFERENCE}
\bibliographystyle{refstyle}
\renewcommand\refname{REFERENCE}


%-------------Li-Ping's Definition-----------------------%
\def\hDash{\bot\!\!\!\bot}
\def\wh{\widehat}
\def\wt{\widetilde}
\def\ba{\mbox{\boldmath$\alpha$}}
\def\bb{\mbox{\boldmath$\beta$}}
\def\bg{\mbox{\boldmath$\gamma$}}
\def\ha{\mbox{$\widehat\ba$}}
\def\hb{\mbox{$\widehat\bb$}}
\def\hg{\mbox{$\widehat\bg$}}
\def\hDash{\bot\!\!\!\bot}


\def\a{{\bf a}}
\def\b{{\bf b}}
\def\A{{\bf A}}
\def\B{{\bf B}}
\def\C{{\bf C}}
\def\G{{\bf G}}
\def\X{{\bf X}}
\def\x{{\bf x}}
\def\Y{{\bf Y}}
\def\y{{\bf y}}
\def\Z{{\bf Z}}
\def\z{{\bf z}}
\def\u{{\bf u}}
\def\s{{\bf s}}
\def\t{{\bf t}}
\def\h{{\bf h}}
\def\k{{\bf k}}
\def\l{{\bf l}}
\def\c{{\bf c}}
\def\d{{\bf d}}
\def\w{{\bf w}}
\def\g{{\bf g}}
\def\I{{\bf I}}
\def\R{{\bf R}}
 \def\vo{{\bf 1}}
\def\vz{{\bf 0}}

\def\balpha{{\bm \alpha}}
\def\bbeta{{\bm \beta}}
\def\bzeta{{\bm \zeta}}
\def\betaa{{\bm \eta}}
\def\bome{{\bm \omega}}
\def\bpi{{\bm \pi}}

\newcommand{\trans}{^{\mbox{\tiny{T}}}}
\def\defby{\stackrel{\mbox{\textrm{\tiny def}}}{=}}

\newcommand{\beps}{\mbox{\boldmath $\varepsilon$}}
\newcommand{\bSig}{\mbox{\boldmath $\Sigma$}}
\newcommand{\hSig}{\mbox{$\widehat{\bSig}$}}
\newcommand{\bLam}{\mbox{\boldmath $\Lambda$}}
\newcommand{\hLam}{\mbox{$\widehat{\bLam}$}}
\newcommand{\bOmega}{\mbox{\boldmath $\Omega$}}
\newcommand{\bI}{\mbox{\boldmath $I$}}
\newcommand{\bGam}{\mbox{\boldmath $\Gamma$}}

\newtheorem{defi}{\sc Definition}[section]
\newtheorem{theo}{\bf Theorem}
\newtheorem{lemm}{\sc Lemma}
\newtheorem{prop}{\sc Proposition}
\newtheorem{coll}{\sc Corollary}[theo]
\newtheorem{rema}{\bf Remark}
\newtheorem{exam}{\bf Example}



\def\diamondplus{\mathrel{%
		\ooalign{\raise.29ex\hbox{$\scriptscriptstyle+$}\cr\hss$\diamond$\hss}}}

%--------------------------------------------------------------%


\headsep 6pt
\topmargin 0in
\textheight 8.5in
\evensidemargin 0.5in
\oddsidemargin 0.5in
\textwidth 6in
\footskip 18pt


\newtheorem*{non-lemma}{\sc Lemma}
\newtheorem{lemma}{Lemma}
\newtheorem{theorem}{Theorem}


\newcommand{\skipline}{\vspace{12pt}}
\newcommand{\Rcor}{{\rm{Rcor}}}
\newcommand{\Scor}{{\rm{Scor}}}
\newcommand{\Dcov}{{\rm{Dcov}}}
\newcommand{\GDcov}{{\rm{GDcov}}}
\newcommand{\Pcov}{{\rm{Pcov}}}
\newcommand{\KAcov}{{\rm{KAcov}}}
\newcommand{\DC}{{{\rm DC}}}
\newcommand{\PC}{{{\rm PC}}}
\newcommand{\KAC}{{{\rm KAC}}}
\newcommand{\BPC}{{{\rm BPCor}}}
\newcommand{\PCPR}{{{\rm PCPR}}}
\newcommand{\HSIC}{{{\rm HSIC}}}

\newcommand{\D}{\mbox{D}}
\newcommand{\E}{\mbox{E}}
\newcommand{\F}{\mbox{F}}
\newcommand{\NLS}{\mbox{NLS}}
\newcommand{\GPLSIM}{\mbox{GPLSIM}}
\newcommand{\Known}{\mbox{Known}}
\newcommand{\PS}{\mbox{PS}}
\newcommand{\PR}{\mbox{PR}}
\newcommand{\LS}{\mbox{LS}}
\newcommand{\LSR}{\mbox{LSR}}
\newcommand{\PPR}{\mbox{PPR}}
\newcommand{\SIR}{\mbox{SIR}}
\newcommand{\pHd}{\mbox{pHd}}
\newcommand{\tr}{\mbox{tr}}
\newcommand{\vech}{\mbox{vech}}
\newcommand{\mvz}{\mbox{${\bf z}$}}
\newcommand{\Hessian}{\mbox{${\bf H}$}}

\newcommand{\ang}{{\rm{ang}}}


\newcommand{\yvec}{\mbox{\boldmath $y$}}

\newcommand{\Zvec}{\mbox{\boldmath $Z$}}
\newcommand{\avec}{\mbox{\boldmath $a$}}
\newcommand{\bvec}{\mbox{\boldmath $b$}}
\newcommand{\mvec}{\mbox{\boldmath $m$}}
\newcommand{\svec}{\mbox{\boldmath $s$}}
\newcommand{\tvec}{\mbox{\boldmath $t$}}
\newcommand{\uvec}{\mbox{\boldmath $u$}}
\newcommand{\wvec}{\mbox{\boldmath $w$}}
\newcommand{\gammavec}{\mbox{\boldmath $\gamma$}}
\newcommand{\epsvec}{\mbox{\boldmath $\epsilon$}}
\newcommand{\zetavec}{\mbox{\boldmath $\zeta$}}
\newcommand{\etavec}{\mbox{\boldmath $\eta$}}
\newcommand{\thetavec}{\mbox{\boldmath $\theta$}}
\newcommand{\chivec}{\mbox{\boldmath $\chi$}}
\newcommand{\Covmat}{\mbox{\boldmath $\Sigma$}}
\newcommand{\Bmat}{\mbox{${\bf B}$}}
% \newcommand{\norm}{\|} % commented by ccy
\usepackage{latexsym}
\usepackage{epsfig}
\usepackage{bm}

\usepackage{threeparttable}
\usepackage{booktabs}
%\usepackage{siunitx,booktabs} % table row space
%\sisetup{separate-uncertainty}
%\renewcommand{\baselinestretch}{1.75}
%
%\newcommand{\csection}[1]
%{\begin{center}
%		\stepcounter{section}
%		{\bf\large\arabic{section}. #1}
%	\end{center}
%	\vspace{-0.15 cm}}
%\newcommand{\scsection}[1]
%{\begin{center}
%		{\bf\large #1}
%	\end{center}
%	\vspace{-0.15 cm}}
%\newcommand{\csubsection}[1]{
%	\vspace{-0.25 cm}
%	\begin{center}
%		\stepcounter{subsection}
%		{\it\arabic{section}.\arabic{subsection}. #1}
%	\end{center}
%	\vspace{-0.25 cm}}
%\newcommand{\scsubsection}[1]{
%	\vspace{-0.25 cm}
%	\begin{center}
%		\stepcounter{subsection}
%		{\it #1}
%	\end{center}
%	\vspace{-0.25 cm}}
%
%
%
%
%%\usepackage{xr}
%%\externaldocument{其他文件名称，可以引用其他文件中出现的标号} % 例如，
%\usepackage{xr}
%\externaldocument{chap1}
%% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %
%%                      																								  %
%%                      					可能需要使用特殊的一些包    			    			 %
%%                      																								  %
%% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %
%\RequirePackage[mathlines, displaymath]{lineno}
%\usepackage{natbib}
%\usepackage{latexsym, amsbsy, amssymb,multirow, epsfig, amsmath}
%\usepackage[left=30mm,right=28mm,top=2cm,bottom=2cm]{geometry}
%%\usepackage{amssymb,amsthm,amsmath,mathrsfs,bm,color}
%%\setlength{\textwidth}{6.2in} \setlength{\textheight}{8.75in}
%%\setlength{\topmargin}{-0.25in} \setlength{\oddsidemargin}{0.25in}
%%\setlength{\evensidemargin}{0.25in}
%%\usepackage{hyperref}
%%\baselineskip = 7mm
%%\parskip = 2.5mm
%%
%%\textheight= 9in
%%\textwidth = 6.1in
%%\evensidemargin = 0in
%%
%
%
%% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %
%%                      																								  %
%%                      					可能需要使用特殊的命令行    			    			 %
%%                      																								  %
%% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %
%\def\beqr{\begin{eqnarray}}
%\def\eeqr{\end{eqnarray}}
%\def\beqrs{\begin{eqnarray*}}
%\def\eeqrs{\end{eqnarray*}}
%
%% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %
%%                      																								  %
%%                      					给出比较常用的定理环境定义  	   	   	    			 %
%%                      																								  %
%% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %
%\newtheorem{theo}{\bf Theorem}
%\bibliographystyle{refstyle}
%\renewcommand\refname{REFERENCE}
%
%% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %
%%                      																								  %
%%                      					给出比较常用的特殊算子定义  		   	    			 %
%%                      																								  %
%% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %
%\def\pr{\mbox{pr}}
%\def\cov{\mbox{cov}}
%\def\var{\mbox{var}}
%\def\sign{\mbox{sign}}
%\def\sp{\textrm{span}}
%\def\vecl{\textrm{vecl}}
%
%
%
%% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %
%%                      																								  %
%%                      					给出比较常用的特殊符号定义  		   	    			 %
%%                      																								  %
%% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %
%\def\mR{\mathbb{R}}
%\def\calA{\mathcal{A}}
%\def\calB{\mathcal{B}}
%\def\calC{\mathcal{C}}
%\def\calD{\mathcal{D}}
%\def\calI{\mathcal{I}}
%\def\calN{\mathcal{N}}
%\def\calS{\mathcal{S}}
%\def\calX{\mathcal{X}}
%\def\calY{\mathcal{Y}}
%\def\calZ{\mathcal{Z}}
%
%
%\def\a{{\bf a}}
%\def\b{{\bf b}}
%\def\c{{\bf c}}
%\def\d{{\bf d}}
%\def\u{{\bf u}}
%\def\v{{\bf v}}
%\def\w{{\bf w}}
%\def\x{{\bf x}}
%\def\y{{\bf y}}
%\def\z{{\bf z}}
%
%\def\A{{\bf A}}
%\def\B{{\bf B}}
%\def\C{{\bf C}}
%\def\D{{\bf D}}
%\def\I{{\bf I}}
%\def\X{{\bf X}}
%\def\Y{{\bf Y}}
%\def\Z{{\bf Z}}
%
%
%\def\ba{\mbox{\boldmath$\alpha$}}
%\def\bb{\mbox{\boldmath$\beta$}}
%\def\bSig{\mbox{\boldmath$\Sigma$}}
%
%% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %
%%                      																								  %
%%                      					给出其他一些的特殊算子定义  		   	    			 %
%%                      																								  %
%% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %
%\def\defby{\stackrel{\mbox{\textrm{\tiny def}}}{=}}
%\newcommand{\trans}{^{\mbox{\tiny{T}}}}
%\def\hDash{\bot\!\!\!\bot}
%\def\wh{\widehat}
%\def\wt{\widetilde}



% --------------- Added by ccy ----------------------- %
% norm & abs
\newcommand{\norm}[1]{\Vert#1\Vert}
\newcommand{\Norm}[1]{\left\Vert#1\right\Vert}
\newcommand{\inner}[2]{\langle #1, #2 \rangle}
\newcommand{\Inner}[2]{\left\langle #1, #2 \right\rangle}
\newcommand{\abs}[1]{\vert#1\vert}
\newcommand{\Abs}[1]{\left\vert#1\right\vert}


\usepackage{enumitem} % redefine enumerate


\usepackage[colorinlistoftodos]{todonotes} % for todo

\usepackage{tikz}

\usepackage{amssymb}


\usepackage{threeparttable}
\usepackage{multirow}

% for caption below table, cf. https://latex.org/forum/viewtopic.php?t=5572.
\usepackage{caption}


\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}

\DeclareMathOperator\supp{supp}


